Images in Sentences: Scaling Interleaved Instructions for Unified Visual Generation

While recent advancements in multimodal language models have enabled image generation from expressive multi-image instructions, existing methods struggle to maintain performance under complex interleaved instructions. This limitation stems from the structural separation of images and text in current paradigms, which forces models to bridge difficult long-range dependencies to match descriptions with visual targets. To address these challenges, we propose \texttt{I}mages i\texttt{N} \texttt{SE}n\texttt{T}ences (\textit{a.k.a}, INSET), a unified generation model that seamlessly embeds images as native vocabulary within textual instructions. By positioning visual features directly at their corresponding semantic slots, INSET leverages the contextual locality of transformers for precise object binding, effectively treating images as dense, expressive language tokens. Furthermore, we introduce a scalable data engine that synthesizes 15M high-quality interleaved samples from standard image and video datasets, utilizing VLMs and LLMs to construct rich, long-horizon sequences. Evaluation results on InterleaveBench demonstrate that INSET significantly outperforms state-of-the-art methods in multi-image consistency and text alignment, with performance gaps widening as input complexity increases. Beyond standard generation, our approach inherently extends to multimodal image editing, integrating visual content as part of the instruction to facilitate highly expressive and creative visual manipulations.

==> tables/interleavebench.tex <==
\begin{table}[htbp]
\centering
\caption{
\textbf{Selected Examples of InterleaveBench: Instructions, Image Assets, and Evaluation Questions.}
}
\label{tab:interleavebench}
\small
\renewcommand{\arraystretch}{1.5} % 增加行间距以提高可读性
\begin{tabular}{|p{5.5cm}|p{4cm}|p{6cm}|}
\hline
\textbf{Instructions} & \textbf{Images} & \textbf{Questions} \\
\hline
A vibrant summer poolside scene under a bright blue sky with fluffy white clouds, where \textbf{anime man} with sunglasses relaxes on \textbf{flamingo float} in crystal clear water. The scene includes colorful beach towels spread on the poolside, a small table with tropical drinks, and distant palm trees swaying gently in the breeze, creating a cheerful vacation atmosphere. & 
\textbf{anime man}: human/06\_anime man.jpg \newline 
\textbf{flamingo float}: object/10\_flamingo float.jpg & 
1. Is there an anime man in the image? \newline 2. Is the anime man wearing sunglasses? \newline 3. Is the anime man in a relaxed state? \newline 4. Is the anime man on the flamingo float? \newline 5. Is the anime man facing the poolside? \newline 6. Is there a flamingo float in the image? \newline 7. Is the flamingo float in the pool water? \newline ...\\
\hline
A warm summer evening scene featuring a \textbf{man} with a relaxed posture standing on the wooden porch of a \textbf{wooden house}, holding a \textbf{cocktail} in his hand. The golden hour sunlight creates a cozy atmosphere as the man enjoys his drink while looking out at the sunset over distant hills. & 
\textbf{man}: human/01\_man.jpg \newline 
\textbf{wooden house}: object/45\_wooden house.jpg \newline 
\textbf{cocktail}: object/63\_cocktail.jpg & 
1. Is there a man in the image? \newline 2. Is the man's posture relaxed? \newline 3. Is the man standing? \newline 4. Is the man on the wooden porch? \newline 5. Is the man holding a cocktail? \newline 6. Is the man looking at the sunset? \newline 7. Is the house made of wood? \newline 8. Does the house have a wooden porch? \newline 9. Is the cocktail in a glass? \newline ...\\
\hline
A casual outdoor scene featuring a \textbf{man} standing in a sunlit park, wearing a vibrant blue \textbf{t-shirt} and holding \textbf{headphones} around his neck. He has a playful expression while holding \textbf{poke ball} in his right hand, with trees and a clear blue sky in the background. A backpack rests beside him on a park bench, suggesting he's enjoying a leisurely afternoon. & 
\textbf{man}: human/08\_man.jpg \newline 
\textbf{t-shirt}: object/41\_t-shirt.jpg \newline 
\textbf{headphones}: object/55\_headphones.jpg \newline 
\textbf{poke ball}: object/54\_Poke Ball.jpg & 
1. Is there a man in the image? \newline 2. Is the man standing? \newline 3. Does the man have a playful expression? \newline 4. Is the man wearing a blue t-shirt? \newline 5. Is the man holding headphones around his neck? \newline 6. Is the man holding a poke ball in his right hand? \newline 7. Is the t-shirt blue? \newline 8. Is the poke ball spherical in shape? \newline 9. Is the poke ball clearly visible? \newline ...\\
\hline
A vibrant city street scene at dusk, where a \textbf{man} stands beneath the warm glow of a \textbf{street lamp}. He wears a \textbf{cap} turned slightly to the side and carries a leather messenger bag over his shoulder. Nearby, a \textbf{hat} rests on a wrought iron bench beside a newspaper. In the background, a \textbf{yellow taxi} drives past, its headlights cutting through the soft evening haze as pedestrians stroll along the sidewalk lined with shops and cafes. & 
\textbf{man}: human/07\_man.jpg \newline 
\textbf{street lamp}: object/15\_street lamp.jpg \newline 
\textbf{cap}: object/32\_cap.jpg \newline 
\textbf{hat}: object/01\_hat.jpg \newline 
\textbf{yellow taxi}: object/44\_yellow taxi.jpg & 
1. Is there a man in the image? \newline 2. Is the man standing beneath the street lamp? \newline 3. Is the man wearing a cap? \newline 4. Is the street lamp emitting a warm glow? \newline 5. Is the cap turned slightly to the side? \newline 6. Is the hat resting on the wrought iron bench? \newline 7. Is there a yellow taxi in the background? \newline 8. Are the taxi's headlights on? \newline 9. Is the taxi driving? \newline ...\\
\hline
\end{tabular}
\end{table}
